Benchmarking Knowledge Editing using Logical Rules

Large Language Models (LLMs) are increasingly deployed in real-world applications that require access to up-to-date knowledge. However, retraining LLMs is computationally expensive. Therefore, knowledge editing techniques are crucial for maintaining current information and correcting erroneous assertions within pre-trained models. Current benchmarks for knowledge editing primarily focus on recalling edited facts, often neglecting their logical consequences. To address this limitation, we introduce a new benchmark designed to evaluate how knowledge editing methods handle the logical consequences of a single fact edit. Our benchmark extracts relevant logical rules from a knowledge graph for a given edit. Then, it generates multi-hop questions based on these rules to assess the impact on logical consequences. Our findings indicate that while existing knowledge editing approaches can accurately insert direct assertions into LLMs, they frequently fail to inject entailed knowledge. Specifically, experiments with popular methods like ROME and FT reveal a substantial performance gap, up to 24%, between evaluations on directly edited knowledge and on entailed knowledge. This highlights the critical need for semantics-aware evaluation frameworks in knowledge editing.

==> Tables/MQuAKE-results.tex <==
 \begin{table*}[t!]
  \small
   
  \begin{center}
   \begin{tabular}{|p{2cm}|p{5cm}|p{2cm}|p{2cm}|}
    \hline
      \textbf{Methods}  & \textbf{Models} & \textbf{F1} & \textbf{em} \\
     \hline

      \multirow{3}{4em}{ROME} & EleutherAI\_gpt-j-6B &  & \\
      & gpt2-medium &  &  \\
      & gpt2-large &  & \\
      \hline
        \multirow{3}{4em}{FT} & EleutherAI\_gpt-j-6B\_constr &  & \\
      & EleutherAI\_gpt-j-6B\_unconstr &  &  \\
      & gpt2-medium\_constr &  & \\
      & gpt2-large\_constr &  & \\
      \hline
      \multirow{1}{4em}{KN} & gpt2-xl &  &  \\
      
    
    
    \hline
   \end{tabular}
   \vspace{4mm}
 \caption{We provide the results of METs evaluation on questions answering pairs generated based on logic rules from MQuAKE dataset for each LLM along with their overall F1 score and Exact Match}
     \vspace{-8mm}
   \label{tab:MQuAKE results}
   \end{center}
 \end{table*}
